Modeling Uncertainty and Using Post-fusion as Fallback Improves Retrieval Augmented Generation with LLMs

The integration of retrieved passages and large language models (LLMs), such as ChatGPTs, has significantly contributed to improving open-domain question answering. However, there is still a lack of exploration regarding the optimal approach for incorporating retrieved passages into the answer generation process. This paper aims to fill this gap by investigating different methods of combining retrieved passages with LLMs to enhance answer generation. We begin by examining the limitations of a commonly-used concatenation approach. Surprisingly, this approach often results in generating "unknown" outputs, even when the correct document is among the top-k retrieved passages. To address this issue, we explore four alternative strategies for integrating the retrieved passages with the LLMs. These strategies include two single-round methods that utilize chain-of-thought reasoning and two multi-round strategies that incorporate feedback loops. Through comprehensive analyses and experiments, we provide insightful observations on how to effectively leverage retrieved passages to enhance the answer generation capability of LLMs.

==> Table/table_top20.tex <==
\clearpage
\begin{table*}[ht]
\centering
\resizebox{1\linewidth}{!}{
\renewcommand{\arraystretch}{1}
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
                & \multicolumn{4}{c}{NQ}           & \multicolumn{4}{c}{TriviaQA}     & \multicolumn{4}{c}{SQuAD}          \\ 
                & EM & F1 & \%Unk & \%NM & EM & F1 & \%Unk & \%NM & EM    & F1 & \%Unk & \%NM \\ \hline
Supervised      &  51.4  &  -  &     -    &    -   &  67.6  & -  &     -    &    -    &   56.7    &  -  &     -    &   -           \\ \hline
Comb     & 34.9   & 44.4   &   19.9\%  &   -   & 53.8   &  60.2  &   12.9\%      &  -            &       &    &         &              \\
Separate      & 40.8   &  50.4  &    3.3\%     &   17.3\%    &  51.4  &  57.4  &     3.6\%    &   16.9\%           &       &    &         &              \\ \hline
Prune Prompt     &  39.0  & 50.5   &  6.9\%       &   -    & 51.2   &  58.1  &   5.4\%      &     -         &       &    &         &              \\
Summary      & 40.5   & 53.28   &    5.1\%     &   -      & 50.9   & 58.8   & 5.5\%        &    -          &       &    &         &              \\
Comb+Sep  & 42.9   & 53.84   &   6.5\%       &   1.8\%          &  \textbf{57.1}  & \textbf{64.1}   & \textbf{2.9\%}        &     1.5\%         &       &    &         &              \\
Sep+Comb &  43.2  & 54.5   &    7.4\%     &  0\%   &  54.2  & 61.6   &  3.6\%       &  \textbf{0\%}           &       &    &         &       \\\hline 
 \multicolumn{9}{l}{\textit{Without gold passage}}\\ 
Comb        &  33.4  & 42.8   &  21.7\%  &   -   & 52.6   &  58.9  &   13.5\%      &  -            &  53.1     &  64.9  &   13.6\%      &       -       \\
Separate       & 40.2   & 49.6   &    3.8\%     &   15.8\%    &  50.8  &  56.8  &     4.1\%    &   15.4\%           &     57.1  &  71.2 &     2.1\%    &     4.3\%         \\ \hline
Prune Prompt      &  34.7  & 45.2   &  8.8\%       &   -    & 50.5   &  57.2  &   5.5\%      &     -         &  47.7     & 62.6   &  6.7\%       &     -         \\
Summary         & 35.8   & 48.0   &    7.8\%     &   -      & 49.9   & 58.4   & 5.4\%        &    -          &  50.4     &  67.04  &      4.7\%   &   -           \\
Comb+Sep     & \textbf{40.4}   &   51.5       &   \textbf{3.6\%}   & 1.7\%   &  \textbf{56.2}  & \textbf{63.2}   &   \textbf{3.4\%}  &  1.1\%       &  60.6     & 74.0   &    1.7\%     &    0.2\%          \\
Sep+Comb &  39.8  & \textbf{51.7}   &    3.8\%     &   \textbf{0\%}   &  53.3  & 60.9   &  4.0\%       & \textbf{ 0\%}           &  63.9     &  76.9  &   2.1\%      &  0\%     \\
\bottomrule
\end{tabular}
}
\caption{Exact match (EM) and F1 scores on filted dev split of the NQ, TriviaQA and SQuAD using Top-20 passages. \%Unk means the percentage of Unknown of answer. \%NM means the percentage of answer Not in Majority.}
\label{tb_20psg}
\end{table*}
